Learning by Transference: Training Graph Neural Networks on Growing Graphs

Graph neural networks (GNNs) use graph convolutions to exploit network invariances and learn meaningful feature representations from network data. However, on large-scale graphs convolutions incur in high computational cost, leading to scalability limitations. Leveraging the graphon -- the limit object of a graph -- in this paper we consider the problem of learning a graphon neural network (WNN) -- the limit object of a GNN -- by training GNNs on graphs sampled from the graphon. Under smoothness conditions, we show that: (i) the expected distance between the learning steps on the GNN and on the WNN decreases asymptotically with the size of the graph, and (ii) when training on a sequence of growing graphs, gradient descent follows the learning direction of the WNN. Inspired by these results, we propose a novel algorithm to learn GNNs on large-scale graphs that, starting from a moderate number of nodes, successively increases the size of the graph during training. This algorithm is further benchmarked on a decentralized control problem, where it retains comparable performance to its large-scale counterpart at a reduced computational cost.

==> TSP - Learning by transference/01-intro.tex <==
	\section{Introduction}
	\label{sec:Intro}
    
    
	Graph neural networks (GNNs) are deep convolutional architectures formed by a succession of layers where each layer composes a graph convolution and a pointwise nonlinearity \cite{9046288,ZHOU202057}. Tailored to network data, GNNs have been used in a variety of applications such as recommendation systems \cite{fan2019graph,tan2020learning,ying2018graph,schlichtkrull2018modeling, ruiz2019invariance} and Markov chains \cite{qu2019gmnn,ruiz2019gated,li2015gated}, and fields such as biology \cite{NIPS2017_f5077839,NIPS2015_f9be311e,pmlr-v70-gilmer17a,chen2020can} and robotics \cite{qi2018learning,gama2021distributed,li2019graph}.
	%Compared to standard Convolutional Neural Networks (CNNs), which impose a fixed structure for the data, GNNs utilize the connectivity graph structure of the data. 
	Their success in these fields and applications provides ample empirical evidence of the ability of GNNs to generalize to unseen data. More recently, their successful performance has also been justified by theoretical works showing that GNNs are invariant to relabelings \cite{chen2019equivalence,keriven2019universal}, stable to graph perturbations \cite{gama2020stability}, transferable across graphs \cite{ruiz2020graphonTransferability}, and expressive \cite{kanatsoulis2022graph}. 

	
	One of the most important features of a GNN is that, since the linear operation is a graph convolution, its number of parameters does not depend on the number of nodes of the graph. In theory, this means that GNNs can be trained on graphs of any size. But if the graph has large number of nodes, in practice training the GNN is costly because computing graph convolutions involves large matrix operations. While this issue could be mitigated by transferability~\cite{ruiz2021transferability}, i.e., by training the GNN on a smaller graph to execute it on the large graph, this approach does not give any guarantees on the distance between the optimal solutions on the small and on the large graph. In other words, when executing the GNN on the target graph we do not know if its error will be dominated by the transferability error or by the generalization error stemming from the training procedure. 
	
%	{One of the most important features of a GNN is that, because the linear operation is a graph convolution, its number of parameters does not depend on the number of nodes of the graph. In theory, this means that GNNs can be trained on graphs of any size. In practice, however, if the graph has large number of nodes training the GNN is costly because computing graph convolutions involves large matrix operations. \textbf{While this issue could be overlooked}, as we are able to train the GNN on a smaller graph to execute on the large graph, we do not have any guarantees on the distance between the optimal solutions on the small and on the large graph. In other words, when executing the GNN on the target graph we do not know if its error will be dominated by the transferability error or by the generalization error from training. }
	
%	\red{Juan is worried that we mention transfer learning but we never compare our method with any other method of the existing literature.}
	
	%In this paper, we address this problem by incorporating transfer learning into the training process of the GNN.
	
	In this paper, we propose a learning technique for training a GNN on a large graph by progressively increasing the size of the network, and we provide the theoretical guarantees under which the GNN converges to its limit architecture. We consider the limit problem of learning an ``optimal'' neural network for a graphon, which is both a graph limit and a random graph model \cite{lovasz2012large,borgs2017graphons,borgs2010moments}.  We postulate that, because sequences of graphs sampled from the graphon converge to it, the so-called graphon neural network \cite{ruiz2020graphonTransferability} can be learned by sampling graphs of growing size and training a GNN on these graphs (Algorithm \ref{alg:WNNL}). We prove that this is true in two steps. In Theorem \ref{thm:grad_Approximation}, we bound the expected distance between the gradient descent steps on the GNN and on the graphon neural network by a term that decreases asymptotically with the size of the graph. A consequence of this bias bound is that it allows us to quantify the trade-off between a more accurate gradient and one that could be obtained with less computational power. We then use this theorem to prove our main result in Theorem \ref{thm:WNN_learning}, which is stated in simplified form below.
	
	%In order to study very large graphs, in this paper we consider the limit object of a series of converging graphs, a graphon. We sample the edges of the graph according to a Bernoulli distribution whose mean is given by the value of the graphon $\bbW$ function. This general framework allows us to characterize a wide variety of stochastic graphs as belonging to the same family of graphs. 
	
	%Leveraging transferability properties of GNNs, this work introduces a learning procedure that progressively increases the size of the graph while training. We provide theoretical guarantees that the learning iterates computed is the graph $\bbG_n$ follow the direction of the gradient on the very large.  Considering a loss function $\ell$ that we try to minimize, we can do local evaluations of the learning direction by computing the gradient on available data. 
	%The main result of this work is to assess the expected difference between the empirical gradient on the graph $\bbG_n$ with $n$ nodes, and limit object, $\bbW$.

 	\textbf{Theorem} (Graphon neural network learning, informal) Let $\bbW$ be a graphon and let $\{\bbG_n\}$ be a sequence of growing graphs sampled from $\bbW$. Consider the graphon neural network $\bbPhi(\bbW)$ and assume that it is learned by training the GNN $\bbPhi(\bbG_n)$ with loss function $\ell(\bby_n,\bbPhi(\bbG_n))$ on the sequence $\{\bbG_n\}$. Over a finite number of training steps, we obtain
 	$$
 	\|\nabla\ell(Y,\bbPhi(\bbW))\| \leq \epsilon \mbox{ with probability } 1.
 	$$
    
     The most important implication of this result is that the learning iterates computed in the sequence of growing graphs follow the direction of the graphon gradient up to a small ball, which provides theoretical support to the proposed training methodology. To further validate our algorithm, we apply it in a numerical experiment where we consider the problem of flocking. Specifically, we train GNNs to learn the actions agents need to take to flock, i.e., to fly with the same velocities while avoiding collisions\cite{tolstaya2020learning}. We compare the results obtained when progressively increasing the number of agents during training and when training is done directly on the large target graph.
     
     \subsection{Related Work}
     
     GNNs are neural information processing architectures for network data that follow from seminal works in deep learning applied to graph theory \cite{bruna2013spectral,NIPS2016_04df4d43,Gori2005ANM,Lu2003LinkbasedC}.  They have been successfully used in a wide variety of statistical learning problems \cite{kipf2016semi,SCARSELLI2018248}, where their good performance is generally attributed to the fact that they exploit invariances present in network data \cite{maron2019invariant,gama2018convolutional,chami2021machine}. More recently, a number of works show that GNNs can be transferred across graphs of different sizes \cite{ruiz2020graphonTransferability,levie2019transferability,keriven2020convergence}. Specifically, \cite{ruiz2020graphonTransferability} leverages graphons to define families of graphs within which GNNs can be transferred with an error that decreases asymptotically with the size of the graph. The papers by \cite{levie2019transferability} and \cite{keriven2020convergence} offer similar results by considering the graph limit to be a generic topological space and a random graph model respectively. In this paper, we use an extension of the transferability bound derived in \cite{ruiz2020graphonTransferability,ruiz2021transferability} to propose a novel learning algorithm for GNNs.
     
    %\red{JUAN BELIEVES THIS PARAGRAPH IS WASTE OF SPACE}The rest of this paper is organized as follows. Section \red{X} discusses related work and Section \red{X} introduces preliminary definitions. Algorithm \red{X} and Theorems \red{X} and \red{Y} are presented in Section \red{X}. Section \red{X} discusses the numerical results and conclusions are presented in Section \red{X}. All proofs, and further definitions are deferred to the supplementary material.

    %Importantly, it suggests a training methodology exploiting the fact that as solutions approach their optimal values, gradients decrease in norm. This allows us to decrease the bias term (i.e. increase $n$) as learning improves the quality of the solution, without the necessity of incurring into costly computations (i.e. large $n$). 
	
	%Thus, alleviating part of the computational burden without compromising the quality of learning.
	
%	\section{Related Work}
%	\label{sec:RelatedWork}
	
%	\red{Above, paper X is my Neurips paper. Paper Y is called Transferability of Spectral Graph Convolutional Neural Networks by Levie et al. Paper Z is called Convergence and Stability of Graph Convolutional Networks on Large Random Graphs by Keriven et al.}
	
%	\red{I think it is not necessary to talk about GNN training unless you find related papers that use a similar strategy to reduce complexity.}
	
	%When training GNNs, a myard of solutions have been posed. To achieve better resilience against adversarial attacks, some solutions focus on robust training procedures.\cite{10.1007/978-3-030-67664-3_24}. Some, rely on randomly selecting a fixed number of nodes to consider at training \cite{pmlr-v48-niepert16}. Other solutions focus on the ATTENTION. While other set of works have... . Other works focus on the possible parallelization of the training procedure. Recently, some mean field results have shed light over the theoretical performance for classification task of GNNs using back propagation\cite{Kawamoto_2019}. In the context of natural language processing, some works have focused on lowering the dimension of the input data \cite{grover2016node2vec}. 

==> TSP - Learning by transference/02-preliminaries.tex <==

\section{Preliminary Definitions}	
\label{sec:Definitions}

%Graph neural networks are information processing architectures that exploit data invariances from an underlying graph structure. In order to construct a GNNs we need to intercalate successive layers of graph convolutions and point-wise non-linearities.

%Graph neural networks exploit graph symmetries to extract meaningful information from network data \cite{8911416,gama2020stability}. 
A graph is represented as a triplet $\bbG_n=(\ccalV,\ccalE,W)$, where $\ccalV$, $|\ccalV|=n$, is the set of nodes, $\ccalE \subseteq \ccalV \times \ccalV$ is the set of edges and $W:\ccalE\to\reals$ is a map assigning weights to each edge. Alternatively, we can also represent the graph $\bbG_n$ by its graph shift operator (GSO) $\bbS_n\in \reals^{n \times n}$, a square matrix that respects the sparsity pattern of $\bbG_n$. Examples of GSOs include the adjacency matrix $\bbA$, the graph Laplacian $\bbL = \diag(\bbA \boldsymbol{1})-\bbA$ and their normalized counterparts \cite{gama2018convolutional}. In this paper we consider undirected graphs $\bbG_n$, so that $\bbS_n$ is always symmetric, and fix $\bbS_n=\bbA/n$. 

\subsection{Graph Convolutions}

Graph data is represented in the form of graph signals. A graph signal $\bbx_n=[x_1,\dots,x_n]^T\in \reals^n$ is a vector whose $i$-th component corresponds to the information present at the $i$-th node of graph $\bbG_n$. A basic data aggregation operation can be defined by applying the GSO $\bbS_n$ to graph signals $\bbx_n$ as
\begin{align}\label{eqn:graph_shift}
\bbz_n=\bbS_n\bbx_n \text{.}
\end{align}
%The resulting signal $x_i$ is such that the data at node $i$ is a weighted average of
{The value of signal $\bbx_n$ at node $i$, $x_i$, is a weighted} average of the information in the $1$-hop neighborhood of $i$, $z_i = \sum_{j \in \ccalN_i} [\bbS_n]_{ij} x_j$, where $\ccalN_i = \{j \ | \ [\bbS_n]_{ij} \neq 0\}$. Information coming from further neighborhoods (e.g., the $k$-hop neighborhood) can be aggregated by successive applications of the GSO (e.g., $\bbS_n^k\bbx_n$).
%Thus, by successively applying the GSO, the information of the nodes spreads across the entire network while respecting the structure of the graph. 

Using this notion of shift\cite{sandryhaila2013discrete}, we can define \textit{graph convolutions}. Explicitly, the graph convolutional filter with coefficients $\bbh=[h_0,\dots,h_{K-1}]$ is defined as a polynomial on the GSO $\bbS_n$,
\begin{equation} \label{eqn:graph_convolution}
\bby_n = \bbh *_{\bbS_n} \bbx_n = \sum_{k=0}^{K-1} h_k \bbS_n^k \bbx_n
\end{equation}
where $\bbx_n, \bby_n \in \reals^N$ are graph signals and $*_{\bbS_n}$ denotes the convolution operation with GSO $\bbS_n$.

Since the adjacency matrix of an undirected graph is always symmetric, the GSO admits an eigendecomposition $\bbS_n = \bbV \bbLam \bbV^H$. The columns of $\bbV$ are the GSO eigenvectors and the diagonal elements of $\bbLam$ are its eigenvalues, which take values between $-1$ and $1$ and are ordered as $-1 \leq \lambda_{-1} \leq \lambda_{-2} \leq \ldots \leq 0 \leq \ldots \leq \lambda_2 \leq \lambda_1 \leq 1$. 
Since the eigenvectors of $\bbS_n$ form an orthonormal basis of $\reals^n$, we can project \eqref{eqn:graph_convolution} onto this basis to obtain the spectral representation of the graph convolution,
\bal \label{eqn:spectral_graph}
h(\lambda) = \sum_{k=0}^{K-1} h_k \lambda^k \text{.}
\eal
%Defining the change of basis operation $\hby = \bbV^H \bby$ and substituting $\bbS = \bbV \bbLam \bbV^H$ in \eqref{eqn:graph_convolution}, we get $\hby = \sum_{k=0}^{K-1} h_k \bbLam^k \hbx = h(\bbLam) \hbx$. 
Importantly, note that \eqref{eqn:spectral_graph} only depends on the $h_k$ and on the eigenvalues of the GSO. {Hence, by} the Cayley-Hamilton theorem, convolutional filters may be used to represent any graph filter with spectral representation $h(\lambda) = f(\lambda)$ where $f$ is analytic \cite{strang1976}.

\subsection{Graph Neural Networks}

Graph neural networks are layered architectures where each layer consists of a graph convolution followed by a pointwise nonlinearity $\rho$.
%, and where each layer's output is the input to the following layer.  
Layer $l$ can output multiple features $\bbx^f_{nl}$, $1 \leq f \leq F_{l}$, which we stack in a matrix $\bbX_l=[\bbx_{nl}^1,\dots,\bbx^{F_l}_{nl}]\in \reals^{n\times F_l}$. Each column of the feature matrix is the value of the graph signal corresponding to feature $f$. To map the $F_{l-1}$ features coming from layer $l-1$ into $F_l$ features, $F_{l-1} \times F_l$ convolutions need to be computed, one per input-output feature pair. Stacking their weights in $K$ matrices $\bbH_{lk}\in \reals^{F_{l-1}\times F_l}$, we may write the $l$-th layer of the GNN as
\begin{equation} \label{eqn:gcn_layer}
\bbX_{l} = \rho \left( \sum_{k=0}^{K-1} \bbS_n^k \bbX_{l-1} \bbH_{lk} \right). 
\end{equation}
The GNN input (i.e., the input of layer $l=1$) is given by $\bbX_0 = \bbX \in\reals^{n \times F_0}$ and, in an $L$-layer GNN, the operation in \eqref{eqn:gcn_layer} is cascaded $L$ times to obtain the GNN output $\bbY = \bbX_L$. In this paper we assume $F_0=F_L =1$ so that $\bbY= \bby_n$ and $\bbX = \bbx_n$. A more concise representation of this GNN can be obtained by grouping all learnable parameters $\bbH_{lk}$ in a tensor $\ccalH=\{\bbH_{lk}\}_{l,k}$ and defining the map $\bby_n=\bbPhi(\bbx_n;\ccalH,\bbS_n)$. %Since each layer $l$ has a correspondent number of features $F_l$, 
Due to the polynomial nature of the graph convolution, the dimensions of the learnable parameter tensor $\ccalH$ are independent from the size of the graph ($K$ is typically much smaller than $n$). Ergo, a GNN trained on a graph $\bbG_n$ can be deployed on a network $\bbG_m$ with $m \neq n$. 

\subsection{Graphons}

%To formalize the sense in which increasing graphs behave, we need to introduce a limit object, and a sense of convergence. 

\begin{figure*}[t]
\centering
\begin{subfigure}{0.22\textwidth}
\centering
\includegraphics[width=3.7cm]{figures/er_50_2}
\caption{50 nodes}
\label{fig:50nodes}
\end{subfigure}
\hspace{0.3cm}
\begin{subfigure}{0.22\textwidth}
\centering
\includegraphics[width=3.7cm]{figures/er_100}
\caption{100 nodes}
\label{fig:100nodes}
\end{subfigure}
\hspace{0.3cm}
\begin{subfigure}{0.22\textwidth}
\centering
\includegraphics[width=3.7cm]{figures/er_200}
\caption{200 nodes}
\label{fig:200nodes}
\end{subfigure}
\hspace{0.3cm}
\begin{subfigure}{0.22\textwidth}
\centering
\includegraphics[width=3.7cm]{figures/er_graphon}
\caption{Graphon}
\label{fig:er_graphon}
\end{subfigure}

\caption{Sequence of stochastic graphs with 50 (a), 100 (b), and 200 nodes (c) converging to the constant graphon (d).}
\label{fig:graphon_example}
\end{figure*}

A graphon is a bounded, symmetric, and measurable function $\bbW:[0,1]^2\to [0,1]$ which has two theoretical interpretations; it is both a graph limit and a generative model for graphs. In the first interpretation, sequences of dense graphs converge to a graphon in the sense that the densities of adjacency-preserving graph motifs converge to the densities of these same motifs on the graphon \cite{lovasz2012large}. A graphical example of the convergence of dense graphs to a graphon is depicted in figure \ref{fig:graphon_example}. In the second, graphs can be generated from a graphon by sampling points $u_i, u_j$ from the unit interval and either assigning weight $\bbW(u_i,u_j)$ to edges $(i,j)$, or sampling edges $(i,j)$ with probability $\bbW(u_i,u_j)$. 
In this paper, we focus on graphs $\bbG_n$ where the points $u_i$ are defined as $u_i = (i-1)/n$ for $1 \leq i \leq n$ and where the adjacency matrix $\bbS_n$ is sampled from $\bbW$ as
\begin{align} \label{eqn:BernoulliSampledGraph}
[\bbS_n]_{ij} &\sim \text{Bernoulli}([\mbS_n]_{ij}),\text{with }{[\mbS_n]_{ij}} = \bbW(u_i,u_j)
\end{align}
We refer to the graph $\bbS_n$ as a \textit{stochastic graph}, and to the graph $\mbS_n$ from which its edges are sampled as the $n$-node \textit{template graph} associated with the graphon $\bbW$. Sequences of stochastic graphs generated in this way can be shown to converge to $\bbW$ with probability one \cite{lovasz2012large}[Chapter 11].

%As the graph increases, so does the granularity of the nodes in the graphon, thus increasing the resemblance between the two. Graphs and graphon admit the dual interpretation, every graphon is the limit object of a convergent graph sequence, and every convergent graph sequence converges to a graphon \cite[Chapter 11]{lovasz2012large}. 

%To formalize the convergence of the graph sequence we introduce graph ``motifs'' $\bbF$ a generic unweighted and undirected graphs $\bbF = (\ccalV^{'},\ccalE^{'})$ with $n^{'}$ nodes. If  motif $\bbF$ has less nodes than graph $\bbG_N$, homomorphisms of $\bbF$ into $\bbG_n$ quantify how many times we can fit the motif into the graph. Formally, homomorphisms are maps that respect the adjacency of the two graphs, i.e. if $(i,j)\in \ccalE^{'}$ then $(i,j)\in \ccalE$.  The total number of maps from $\ccalV^{'}$ into $\ccalV$ is $|\ccalV|^{|\ccalV^{'}|}=n^{n^{'}}$, thought a portion of them are homomorphisms. We can thus quantify the density of homomorphisms $t(\bbG_n, \bbF)$ as the quotient between the actual and the total number of homomorphisms between graph $\bbG_n$, and motif $\bbF$. Homomorphisms of graph motifs $\bbF$ into graphons $\bbW$ are defined in the same way. Putting the pieces together, the convergence of a graph sequence $\{\bbG_n\}$ to a graphon $\bbW$ occurs in homomorphism densities, as follows, 

%\begin{equation} \label{eqn_graphon_convergence}
%\lim_{N\to\infty} t(\bbF,\bbG_n) = t(\bbF,\bbW).
%\end{equation}

In practice, the two theoretical interpretations of a graphon allow thinking of it as an identifying object for a \textit{family} of graphs of different sizes that are structurally similar. Hence, given a network we can use its family's identifying graphon as a continuous proxy for the graph. This is beneficial because it is typically easier to operate in continuous domains than in discrete domains, even more so if the network is large. In the following, we will leverage these ideas to consider graphon data and graphon neural networks as proxies for graph data and GNNs supported on graphs of arbitrary size.

%\begin{align}\begin{split} \label{eqn:det_gcn}
%&[\bar \bbS_n]_{ij} = \bbW(u_i,u_j), \quad \mbox{and} \\
%&[\bar \bbx_n]_i = X(u_i), \quad \mbox{and} \\
%&[\bar \bby_n]_i = Y(u_i).
%\end{split}\end{align}

%	The previous expression \eqref{eqn:det_gcn} shows how to obtain the deterministic graph data from a graphon data. This is particularly important as we will assume our graph data to be generated from a graphon.''} \red{Rewrite the part highlighted in red. Define weighted graphs briefly as an example of graphs that can be generated from graphons, only using in-line equations, as they are not the main type of graph considered in this paper. We will only use actual equations to define stochastic graphs sampled from the graphon, which are the ones we are interested in.} 



==> TSP - Learning by transference/03-WNN.tex <==

\subsection{Graphon Convolutions}

{A graphon signal is defined as a function $X \in L^2([0,1])$. Analogously to graph signals, graphon signals can be diffused by application of a linear} integral operator given by
\begin{equation}
T_{\bbW}X(v) = \int_0^1 \bbW(u,v)X(u)du.
\end{equation}
which we call the graphon shift operator (WSO). Since $\bbW$ is bounded and symmetric, $T_{\bbW}$ Hilbert-Schmidt and self-adjoint \cite{lax02-functional}. As such, $\bbW$ can be written as $\bbW(u,v) = \sum_{i \in \mbZ\setminus\{0\}} \lambda_i \varphi_i(u)\varphi_i(v)$ where $\lambda_i$ are the graphon eigenvalues and $\varphi_i$ the graphon eigenfunctions. The eigenvalues have magnitude at most one and are ordered as $-1 \leq \lambda_{-1} \leq \lambda_{-2} \leq \ldots\leq 0 \leq \ldots \lambda_2 \leq \lambda_1 \leq 1$. The eigenfunctions form an orthonormal basis of $L^2([0,1])$. 

The notion of a graphon shift allows defining graphon convolutions and specifically, we define the graphon convolutional filter with coefficients $[h_0,\dots,h_{K-1}]$ as
\begin{align}\begin{split} \label{eq:graphon_convolution}
&Y =T_\bbh X = \bbh *_{\bbW} X = \sum_{k=0}^{K-1} h_k (T_{\bbW}^{(k)} X)(v) \quad \mbox{with} \\
&(T_{\bbW}^{(k)}X)(v) = \int_0^1 \bbW(u,v)(T_\bbW^{(k-1)} X)(u)du
\end{split}\end{align}
where $X, Y \in \L^2([0,1])$ are graphon signals, $*_{\bbW}$ denotes the convolution operation with graphon $\bbW$ and $T_{\bbW}^{(0)}=\bbI$ is the identity \cite{ruiz2020graphonFourierTransform}.
Projecting the filter \eqref{eqn:graph_convolution} onto the eigenbasis $\{\varphi_i\}_{i \in \mbZ\setminus\{0\}}$, we see that the graphon convolution admits a spectral representation given by
\bal
h(\lambda) = \sum_{k=0}^{K-1} h_k \lambda^k \text{.}
\eal
Like its graph counterpart, the spectral representation of the graphon convolution only depends on the coefficients $\bbh$ and on the eigenvalues of the graphon.  

\subsection{Graphon Neural Networks}

Graphon neural networks (WNNs) are the extensions of GNNs to graphon data. In the WNN, each layer consists of a bank of graphon convolutions \eqref{eq:graphon_convolution} followed by a nonlinearity $\rho$. Assuming that layer $l$ maps $F_{l-1}$ features into $F_l$ features, the parameters of the $F_{l-1} \times F_l$ convolutions \eqref{eq:graphon_convolution} can be stacked into $K$ matrices $\{\bbH_{lk}\}\in \reals^{F_{l-1}\times F_l}$. Then, we can write the $f$th feature of the $l$th layer as 
%\begin{equation}
%X^f_{\ell} = \rho\left(\sum_{g=1}^{F_{\ell-1}} \bbh_{\ell}^{fg} *_\bbW X^g_{\ell-1} \right)
%\end{equation}
\begin{equation}\label{eqn:wcn_layer}
X_{l}^{f} = \rho\left(\sum_{g=1}^{F_{l-1}} \sum_{k=1}^{K-1} (T_{\bbW}^{(k)} X^g_{l-1})[\bbH_{lk}]_{gf} \right)
\end{equation}
for $1 \leq f \leq F_{l}$. 

For an $L$-layer WNN, $X_0^g$ is given by the input data $X^g$ for $1 \leq g \leq F_0$, \eqref{eqn:wcn_layer} is repeated for $1 \leq \ell \leq L$, and the WNN output is given by $Y^f = X_L^f$. In this paper, we fix $F_L=F_0=1$ so that $X_L = Y$ and $X_0 = X$. Like the GNN, the WNN can be represented more succinctly as a map $Y = \bbPhi(X;\ccalH,\bbW)$. The tensor $\ccalH = \{\bbH_{lk}\}_{l,k}$ groups the filter coefficients at all layers and for all features of the WNN. %Note that the parameters in $\ccalH$ are agnostic to the graphon, as they the number of layer $L$, and features per layer $F_l$ are agnostic of the graphon $\bbW$.

%\red{You don't need to make the paragraphs below an independent subsection. You also have to change the order in which you introduce things. First define GNNs sampled from WNNs. GNNs sampled from WNNs are those in which the graph is sampled from the graphon and the graph signal is sampled from the graphon signal. You need to define this first because this is the first concept that you use in Section 4 (see equation 12). In particular, it will make your life easier if in Theorem 1 you can simply say ``consider this WNN and the GNN \textit{sampled from it} on the $n$-node graph $\bbS_n$''. Then, define WNNs induced by GNNs. This is a necessary but much less important definition. You will only need this definition at the end of your theorem statements, after the equation, to clarify that the $\bbPhi(X_n; \ccalH, \bbW_n)$ in the theorem equation is the \textit{WNN induced by the GNN} you sampled on the graph $\bbS_n$.}

%\subsubsection{Sampling GNNs from WNNs}	

From the representation of the GNN and the WNN as maps $\bbPhi(\bbx_n;\ccalH,\bbS_n)$ and $\bbPhi(X;\ccalH,\bbW)$, we see that these architectures can share the same filter coefficients $\ccalH$. this observation is important because, since graphs can be sampled from graphons as in \eqref{eqn:BernoulliSampledGraph}, it implies that we can similarly use the WNN $\bbPhi(X;\ccalH,\bbW)$ to \textit{sample} GNNs
\begin{align} \label{eqn:gcn_obtained}
\bby_n = \bbPhi(\bbx_n;\ccalH,\bbS_n) \mbox{ where }&[\bbS_n]_{ij} \sim \mbox{Bernoulli}(\bbW(u_i,u_j))\nonumber \\
&[\bbx_n]_i = X(u_i) \text{.}
\end{align}
In other words, the WNN can be interpreted as a generative model for GNNs $ \bbPhi(\bbx_n;\ccalH,\bbS_n)$. 

%In particular, when the spectral representation of the graph convolutions $h(\lambda)$ [cf. \eqref{eqn:graph_convolution_spectral}] is such that
%\begin{equation} \label{eqn:constant_filter}
%h(\lambda) = h(c) \mbox{ for } |\lambda| \leq c
%\end{equation}
%for a fixed constant $c \in [0,1]$, GNNs sampled from the WNN as in \eqref{eqn:gcn_obtained} have been shown to approximate the WNN $\bbPhi(X;\ccalH,\bbW)$ arbitrarily well as $n \to \infty$ \red{[cite Luana's NeurIPS and ICASSP papers]}. In Section \ref{sec:WLearning}, we will show that a WNN with convolutional filters satisfying \eqref{eqn:constant_filter} can be learned by training GNNs with the same type of filter on a sequence of increasing graphs.
Conversely, a WNN can be induced by a GNN. Given a GNN $\bby_n = \bbPhi(\bbx_n;\ccalH,\bbS_n)$, the WNN induced by this GNN is defined as 
\begin{align} \label{eqn:wnn_induced}
\begin{split}
Y_n &= \bbPhi(X_n;\ccalH,\bbW_n) \mbox{ where }\\
\bbW_n(u,v) &= \sum_{i=1}^n\sum_{j=1}^n [\bbS_n]_{ij} \mbI(u \in I_i) \mbI(v \in I_j) \\
X_n(u) &= \sum_{i=1}^n [\bbx_n]_i \mbI(u \in I_i)
\end{split}
\end{align}
where $\mbI$ denotes the indicator function and the intervals $I_i$ are defined as $I_i=[(i-1)/n,i/n)$ for $1 \leq i \leq n-1$ and $I_n = [(n-1)/n,1]$. The graphon $\bbW_n$ and the signals $X_n$ and $Y_n$ are respectively the \textit{graphon induced by the graph} $\bbG_n$ and the \textit{graphon signals induced by the graph signals} $\bbx_n$ and $\bby_n$.


==> TSP - Learning by transference/04-WLearning.tex <==
	\section{Graphon Empirical Learning}
	\label{sec:WLearning}
	
	%We live in the era of learning and connectivity, which translates in more gadgets added to the connected network. Previous solutions that rely on graph structures may become obsolete if they are unable to address scalability problems. 
	
	{In this paper, our goal is to solve statistical learning problems where the data is supported on very large graphs. We restrict the optimization domain to the function class of graphon neural networks (cf. \eqref{eqn:wcn_layer}) both to avoid trivial solutions and to be able to generalize to unseen data while leveraging invariances of the graph. Explicitly, we aim to solve an optimization problem of the form}
	
% 	On graphons, the statistical loss minimization (or statistical learning) problem is given by add text}
	\begin{align}\label{eqn:SRM}
	\underset{\ccalH}{\text{minimize}} \quad \mbE_{p(Y,X)}[\ell(Y,\bbPhi(X;\ccalH,\bbW))]
	\end{align}
	where $p(Y,X)$ is an unknown joint data distribution, $\ell$ a {non-negative} loss function and $\bbPhi(X;\ccalH,\bbW)$ a WNN parametrized by the graphon $\bbW$ and by a set of learnable weights $\ccalH$. In this paper, we consider non-negative loss functions $\ell: \reals\times\reals\to\reals^{+}$, such that $\ell(x,y)=0$ if and only if $x=y$. Because the joint probability distribution $p(Y,X)$ is unknown, we cannot derive a closed-form solution of \eqref{eqn:SRM}, but this problem can be approximated by the empirical risk minimization (ERM) problem over graphons.
	
	\subsection{Graphon Empirical Risk Minimization}
	
	 Suppose that we have access to samples of the distribution $\ccalD=\{(X^j,Y^j)\sim p(X,Y), j=1,\dots,|\ccalD|\} $. Provided that these samples are obtained independently and that $|\ccalD|$ is sufficiently large, the statistical loss in \eqref{eqn:SRM} can be approximated by {the empirical sum over $\ccalD$,}
	 	\begin{align}\label{eqn:ERM}
	\underset{\ccalH}{\text{minimize}} \quad \sum_{j=1}^{|\ccalD|}\ell(Y^j,\bbPhi(X^j;\ccalH,\bbW))
	\end{align}
	 giving way to the ERM problem \cite{hastie2009elements,shalev2014understanding,vapnik1999nature,kearns1994introduction}. To solve this problem using local information, we {can use} gradient descent \cite{goodfellow2016deep}. The $k$th gradient descent iteration is given by
	\bal
	\ccalH_{k+1}&=\ccalH_{k}-\eta_k \frac{1}{|\ccalD|}\sum_{j=1}^{|\ccalD|}\nabla_{\ccalH} \ell(Y^j,\bbPhi(X^j;\ccalH_k,\bbW))\label{eqn:WNN_Learning_Step}
	\eal
	where $\eta_k\in (0,1)$ is the step size at iteration $k$. 
	
	In practice, the gradients on the right hand side of \eqref{eqn:WNN_Learning_Step} cannot be computed because the graphon $\bbW$ is an unknown limit object.
	%rendering the graphon learning step \eqref{eqn:WNN_Learning_Step} unimplementable.  
	However, we can exploit the fact that $\bbW$ is a random graph model to approximate the gradients $\nabla_{\ccalH} \ell(Y^j,\bbPhi(X^j;\ccalH,\bbW))$ by sampling stochastic graphs $\bbG_n$ with GSO $\bbS_n$ [cf. \eqref{eqn:BernoulliSampledGraph}] and calculating $\nabla_{\ccalH} \ell(\bby^j_n,\bbPhi(\bbx^j_n;\ccalH,\bbS_n))$, where $\bbx_n^j$ and $\bby_n^j$ are respectively graph signals and graph labels as in \eqref{eqn:gcn_obtained}. In this case, the graphon empirical learning step in \eqref{eqn:WNN_Learning_Step} becomes 
	%However, if the structure of the problem remains unchanged, we can resort to successive evaluations of the graphon, obtaining stochastic graphs $\bbS_n$ respectively .  Hence, the graphon empirical learning step \eqref{eqn:WNN_Learning_Step} can be tailored to its stochastic graph counter part as, 
	\bal
	\ccalH_{k+1}&=\ccalH_{k}-\eta_k  \frac{1}{|\ccalD|}\sum_{j=1}^{|\ccalD|} \nabla_{\ccalH} \ell(\bby^j_{n},\bbPhi(\bbx^j_{n};\ccalH_k,\bbS_n)). \label{eqn:GNN_Learning_Step}
	\eal

	As we show in the next subsection, the gradient descent iterates on the graph \eqref{eqn:GNN_Learning_Step} are good approximations of the gradient descent steps on the graphon \eqref{eqn:WNN_Learning_Step}.
	%The main difference between the graphon empirical learning step \eqref{eqn:WNN_Learning_Step}, and the graph empirical learning step \eqref{eqn:GNN_Learning_Step} is the convolution operator cast in the neural network. 

\subsection{Gradient Approximation}

%In order to learn WNNs using the gradient descent iterates in \eqref{eqn:GNN_Learning_Step}, we need to relate these gradient descent steps with the gradient descent steps on the graphon \eqref{eqn:WNN_Learning_Step}. In the following, we derive an upper bound for the expected error made when using the gradient calculated on the graph to approximate the gradient on the graphon. 
%In what follows, we give a closed-form expression of this bound, and use it as a stepping stone to develop an algorithm that increases $n$, the graph size, at regular intervals during the training process of the GNN. We then prove that our algorithm converges to a neighborhood of the optimal solution for the WNN. 
%analyze the relationship between the two aforementioned gradient. 

In order to derive an upper bound for the expected error made when using the graph gradients \eqref{eqn:GNN_Learning_Step} to approximate the graphon gradients \eqref{eqn:WNN_Learning_Step}, we introduce a Lipschitz smoothness definition, as well as two definitions related to the spectra of the graphon $\bbW$ and the graphon $\bbW_n$ induced by $\bbS_n$ (cf. equation \ref{eqn:wnn_induced}).

%recall the definition of Lipschitz continuity and introduce \textit{normalized} Lipschitz functions.
\begin{definition}[Lipschitz continuous functions] \label{def:norm_lips}
	A function $f(u_1, u_2, \ldots, u_d)$ is $A$-Lipschitz on the variables $u_1, \ldots, u_d$ if it satisfies $|f(v_1,v_2,\ldots,v_d)-f(u_1,u_2,\ldots,u_d)| \leq A\sum_{i=1}^d |v_i-u_i|$.
	If $A=1$, we say that this function is normalized Lipschitz.
\end{definition}
%Consider the GNN $\bbPhi(\bbx_n;\ccalH,\bbS_n)$ instantiated from the WNN $\bbPhi(X;\ccalH,\bbW)$ as in \eqref{eqn:BernoulliSampledGraph} and \eqref{eqn:gcn_obtained}. 
%{The graph and the graphon need to be related, this requires further assumptions.} 

\begin{definition}[$c$-band cardinality of $\bbW$]
\label{def:c_band_cardinality}
{The $c$-band cardinality, denoted $B_{\bbW}^c$, is the number of eigenvalues whose absolute value is larger than $c$, }
\bal
B_{\bbW}^c = \# \{\lambda_i:\|\lambda_i\|\leq c \}\nonumber
\eal
\end{definition}
\begin{definition}[$c$-eigenvalue margin of $\bbW$ - $\bbW_n$]
\label{def:c_eigenvalue_margin}
{The $c$-eigenvalue margin of $\bbW$ and $\bbW_n$ is the minimum distance between eigenvalues $\lambda_i(T_\bbW)$ and $\lambda_j(T_{\bbW_n})$, $i \neq j$, }
\bal
\delta_{\bbW\bbW_n}^c = \min_{i,j\neq i}  \{ \| \lambda_i(T_\bbW) - \lambda_i(T_{\bbW_n})\| : \| \lambda_i(T_{\bbW_n})\|\geq c \}\nonumber
\eal
\end{definition}

We also impose the following Lipschitz continuity assumptions (AS\ref{as1}--AS\ref{as4}), and an assumption on the size of the graph $\bbS_n$ (AS\ref{as5}).

\begin{assumption} \label{as1}
	The graphon $\bbW$ and the graphon signals $X$ and $Y$ are normalized Lipschitz.
\end{assumption} 
\begin{assumption} \label{as2}
	The convolutional filters $h$ are normalized Lipschitz and non-amplifying, i.e., $\|h(\lambda)\|<1$.
\end{assumption} 
\begin{assumption} \label{as3}
	The activation functions and their gradients are normalized Lipschitz, and $\rho(0)=0$.
\end{assumption} 
\begin{assumption} \label{as4}
	The loss function $\ell: \reals\times\reals\to\reals^{+}$ and its gradient are normalized Lipschitz, and $\ell(x,x)=0$.
\end{assumption}
\begin{assumption} \label{as5}
	For a fixed value of $\xi \in (0,1)$, $n$ is such that $n-{\log (2n /\xi)}/{d_\bbW}> {2}/{d_\bbW}$ where $d_\bbW$ denotes the maximum degree of the graphon $\bbW$, i.e., $d_\bbW=\max_v \int^1_0 \bbW(u,v)du$.
\end{assumption} 

Under AS\ref{as1}--AS\ref{as5}, the expected norm of the difference between the graphon and graph gradients in \eqref{eqn:WNN_Learning_Step} and \eqref{eqn:GNN_Learning_Step} is upper bounded by Theorem \ref{thm:grad_Approximation}. The proof is deferred to the Appendix \ref{sec:AppendixA}.

%\red{Talk to Juan about theorem statement. Need to define how to sample GNNs from WNNs in the preliminary definitions (Sec. 3) to simplify the statement. Need to define $\delta_c$ and $B_{c}$. Will we need to introduce weighted graphs to define them? Are the filters constant below a certain $c$? Where is this being specified?}

%\red{I have rewritten the theorem statement. Please see below. We have a bigger problem though, which is that filters that are constant below a certain $c$ can never be written as graph convolutions, yet we assume them to be convolutional. If we remove the requirement that these filters be constant below a certain $c$, the transferability bound has an extra term proportional to $c\|X\|$ which does not disappear as we increase $n$. Would Theorems 1 and 2 hold if the transferability theorem had this extra term?}	

\begin{theorem}\label{thm:grad_Approximation}
	%(Graph to Graphon Learning Step Approximation).
	Consider the ERM problem in \eqref{eqn:ERM} and let $\bbPhi(X;\ccalH,\bbW)$ be an $L$-layer WNN with $F_0=F_L=1$, and $F_{l}=F$ for $1\leq l \leq L-1$.  Let $c \in (0,1]$ and assume that the graphon convolutions in all layers of this WNN have $K$ filter taps [cf. \eqref{eq:graphon_convolution}]. Let $\bbPhi(\bbx_n;\ccalH,\bbS_n)$ be a GNN sampled from $\bbPhi(X;\ccalH,\bbW)$ as in \eqref{eqn:gcn_obtained}. Under assumptions AS\ref{as1}--AS\ref{as5}, it holds
	\bal\label{eq:thm_1}
	\mbE[\|\nabla_{\ccalH}&\ell(Y,\bbPhi(X;\ccalH,\bbW))-\nabla_{\ccalH}\ell(Y_n,\bbPhi(X_n;\ccalH,\bbW_n))\|]\nonumber\\
	&\leq \gamma c+\ccalO\bigg( \sqrt{\frac{\log(n^{3/2})}{n}}\bigg)
	%3L^2F^{2L-2}\bigg( 1+\frac{\pi B^{c}_{\bbW \bbW_n}}{\delta_{\bbW \bbW_n}^c}\bigg)\sqrt{\frac{\log (2n^{3/2})}{n}}+12L^2F^{2L-2}c \label{eq:thm_1}
	\eal
	where $Y_n$ is the graphon signal induced by $[\bby_n]_i = Y(u_i)$ [cf. \eqref{eqn:wnn_induced}], and $\gamma$ is a constant that depends on the number of layers $L$, features $F$, and filter taps $K$ of the GNN [cf. Definition \ref{def:Constant_Of_GNN} in the Appendix \ref{sec:AppendixA}]. %The fixed constants $B^c_{\bbW}$ and $\delta^c_{\bbW \bbW_n}$ are the $c$-band cardinality and the $c$-eigenvalue margin of $\bbW$ and $\bbW_n$ respectively [cf. Definitions \ref{def:c_band_cardinality},\ref{def:c_eigenvalue_margin} in the supplementary material].
\end{theorem}
% 	\begin{proof}
% 		See Appendix \ref{sec:AppendixA}.
% 	\end{proof}
% \begin{figure*}[t]
% 	\centering
% 	\input{figures/drawing/gradient.tex}
% 	\caption{In order to satisfy the property that the inner product between the gradient on the GNN $\nabla_{\ccalH}\ell(Y_n,\bbPhi(X_n;\ccalH,\bbW_n))$ and the gradient on the graphon $\nabla_{\ccalH}\ell(Y,\bbPhi(X;\ccalH,\bbW))$ is positive, we rely on the condition provided in Theorem \ref{thm:grad_Approximation} to bound the expected distance between the two gradients. }
% 	\label{fig:grad_ball}
% \end{figure*}
% With respect to assumption \ref{as6}, far from being a limitation, it is an extra layer of information provided for the bound. It allows us to set the minimum number of nodes $n$ from which the Theorem holds true.	
Theorem \ref{thm:grad_Approximation} upper bounds the distance between the learning step on the graph and on the graphon {for a given input-output pair $(X,Y)\in\ccalD$} as a function of the size of the graph. Note that this bound is controlled by two terms.
%: a term that decreases with $n$, and one that is constant.
The first term decreases with $n$ and is an \textit{approximation bound} related to the approximation of $\bbW$ by $\bbS_n$. The second term is a constant \textit{nontransferable bound} controlled by $c$ and related to a threshold that we impose on the convolutional filter $h$. Since graphons $\bbW$ have an infinite spectrum that accumulates around zero, we can only show convergence of all of the spectral components of $Y_n$ in the limit \cite{ruiz2020graphonTransferability}. Given that $n$ is finite, we can only upper bound distances between spectral components associated with eigenvalues larger than some fixed threshold $c \in (0,1]$. The perturbations associated with the other spectral components are controlled by bounding the variation of the filter response below $c$.  %The value of $c$ determines $B_{\bbW \bbW_n}^c$, which counts the number of eigenvalues of $\bbS_n$ larger than $c$; and $\delta_{\bbW \bbW_n}^c$, which is approximately equal to the minimum distance between eigenvalues of $\bbW$ above $c$ [cf. Definitions \ref{def:c_band_cardinality},\ref{def:c_eigenvalue_margin} in the supplementary material]. 

The bound in Theorem \ref{thm:grad_Approximation} is important because it allows us to quantify the error incurred by taking gradient steps not on the graphon, but on the graph data. This is instrumental for learning a meaningful solution of the graphon ERM problem \eqref{eqn:ERM}. Although we cannot calculate gradients of the function that we want to learn [cf. \eqref{eqn:WNN_Learning_Step}], Theorem \ref{thm:grad_Approximation} shows that we can expect to follow the direction of the gradient on the WNN by measuring the ratio between the norm of the gradient of the loss on the GNN and the difference between the two gradients.
%being able to follow the direction of these gradients 
Note however that we are only able to decrease this approximation bound down to the value of the nontransferable bound $\gamma c$. %While we could decrease the nontransferable bound by decreasing $c$, this slows convergence due to the increase of $B_{\bbW \bbW_n}^c$ and the decrease of $\delta_{\bbW \bbW_n}^c$.

%The first set of constants, $\sqrt{K}LF^{3L}$, is related to the total number of hyperparameters $\ccalH$. The term $1+\frac{2\pi n_c^{(q)}}{\delta_c^{(pq)}}\sqrt{\frac{\log\left(2n^{3/2}\right)}{n}}$ is a concentration bound encoding the proximity between a stochastic graph filter and the deterministic one. \red{Do not use frac for in-line equations. Maybe parse these terms in more detail. You never introduced deterministic filters.} This bound is closely related to \cite{chung2011spectra}[Theorem 1]. \red{Not really.} Finally, the bound also depends on the norm and on the energy of the signal on the graphon $X$. \red{Briefly discuss meaning of $B_c$ and $\delta_c$ and their implications.}

\begin{remark}[Feasibility of assumptions] 
AS\ref{as1}--AS\ref{as4} are normalized Lipschitz smoothness conditions which can be relaxed by making the Lipschitz constant greater than one. AS\ref{as3} holds for most activation functions used in practice, e.g., the ReLU and the sigmoid . AS\ref{as4} can be achieved by normalization and holds for most loss functions in a closed set (e.g., the hinge or mean square losses). AS\ref{as5} is necessary to guarantee a $\ccalO(\sqrt{\log{n}/n})$ rate of convergence of $\bbS_n$ to $\bbW$ \cite{chung2011spectra}.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% Section Training on Growing Graphs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{Training on Growing Graphs}

%as a stepping stone towards building the conditions under which we can converge to the graphon neural network. That is, how to assure the convergence of the limit object by following the iterates sampled from it.

%\subsection{Algorithm Construction}
%\label{sec:Algorithm}

An insightful observation that can be made from Theorem \ref{thm:grad_Approximation} is that, since the discretization error depends on the number of nodes of the graph, it is possible to reduce its effect by iteratively increasing the graph size at regular intervals during the training process. In Algorithm \ref{alg:WNNL}, we propose a training procedure that does so at every epoch.
%every epoch. This is what we propose to do in Algorithm \ref{alg:WNNL}. 
% \red{L: The next sentences could use some rewriting/proofreading. Specifically, explain better what is the bias term, and how it is decreased as $k$ increases.} Juan believes thet can be removed allorgether.

% Even if a bias is introduced in the gradient, we will be able to follow the gradient direction of the graphon learning problem \eqref{eqn:WNN_Learning_Step}. 

% At the same time, we need to keep the computational cost of the iterates under control. Note that the norm of the gradient is large at first, but it decreases as we approach the optimal solution. 

% Exploiting this behavior, we may progressively reduce the bias term as iterations increase. 

% The idea here is to keep the discretization of the gradient small so as to closely follow the gradient direction of the graphon learning problem, without however being too conservative---as this would incur in a higher than necessary computational cost. 



\begin{algorithm}[t]
		\caption{Learning by transference}
		\label{alg:WNNL}
		\begin{algorithmic}[1]
			\State   Initialize $\ccalH_0,n_0$ and sample graph $\bbG_{n_0}$ from graphon $\bbW$
			\Repeat \ for epochs $0,1,\ldots$
			\For {$k$ =1,\dots, $|\ccalD|$}
			\State Obtain sample $(Y,X)\sim \ccalD$
			\State Construct graph signal $\bby_n,\bbx_n$ [cf. \eqref{eqn:gcn_obtained}]
			\State Take learning step:\\ \quad\quad\quad\quad$\ccalH_{k+1}=\ccalH_{k}-\eta_k\nabla \ell(\bby_n,\bbPhi(\bbx_n;\ccalH_k,\bbS_n))$
			\EndFor
			\State {Increase number of nodes $n$}
			\State {Sample $\bbS_n$ Bernoulli from graphon $\bbW$ [cf. \eqref{eqn:BernoulliSampledGraph}]}
			\Until  convergence
		\end{algorithmic}
\end{algorithm}

In practice, in the ERM problem the number of nodes that can be added is upper bounded by the maximum graph size in the dataset. As long as we stay under this limit, we can decide which and how many nodes to consider for training arbitrarily. The novelty of Algorithm \ref{alg:WNNL} is that it does not require using the largest available graph to train the GNN. Instead, we can set a minimum graph size $n_0$ and progressively increase it up to the total number of nodes. {The main advantage of Algorithm \ref{alg:WNNL} is thus that it allows reducing the computational cost of training the GNN without compromising its performance. 

{A bound on the difference between the gradients does not, however, imply that we can follow the gradient on the graph blindly. In other words, the fact that gradients are close does not imply that the direction that the iterates follow in the graphon and the graph is the same. In the following subsection, we will thus use Theorem \ref{thm:grad_Approximation} to obtain the conditions under which the gradient steps taken on the graph follow the learning direction we would expect to follow on the graphon, so that Algorithm \ref{alg:WNNL} converges to a neighborhood of the optimal solution on the graphon.

\subsection{Algorithm Convergence}

{To prove that Algorithm \ref{alg:WNNL} converges, we need the following Lipschitz assumption on the neural network and its gradients.}

\begin{assumption} \label{as7}
	The graphon neural network $ \bbPhi(X;\ccalH,\bbW)$ is $\AWNN$-Lipschitz, and its gradient $ \nabla_\ccalH\bbPhi(X;\ccalH,\bbW)$ is $\AgWNN$-Lipschitz, with respect to the parameters $\ccalH$ [cf. Definition \ref{def:norm_lips}].
\end{assumption}

We also need the following lemma that we prove in Appendix \ref{sec:AppendixB}.
\begin{lemma}\label{lemma:martingale}
		%Consider t$\sum \eta_k =\infty$,$\sum \eta_k^2 \leq\infty$. Under Assumptions \ref{as1}-\ref{as7}, if the loss $\ell(Y_n,\Phi(\bbW_n,X_n))$ converges to a finite value, and the.
		Consider the ERM problem in \eqref{eqn:ERM} and let $\bbPhi(X;\ccalH,\bbW)$ be an $L$-layer WNN with $F_0=F_L=1$, and $F_{l}=F$ for $1\leq l \leq L-1$. Let $c \in (0,1]$, $\epsilon>0$, step size $\eta<{\Anl^{-1}}$, with $\Anl=\AnWNN+\AWNN F^{2L} \sqrt{K}$  and assume that the graphon convolutions in all layers of this WNN have $K$ filter taps [cf. \eqref{eq:graphon_convolution}]. Let $\bbPhi(\bbx_n;\ccalH,\bbS_n)$ be a GNN sampled from $\bbPhi(X;\ccalH,\bbW)$ as in \eqref{eqn:gcn_obtained}. Consider the iterates generated by equation \eqref{eqn:GNN_Learning_Step}. Under Assumptions AS\ref{as1}-AS\ref{as7}, if at step $k$ the number of nodes $n$ verifies
		\begin{align}
	      \mbE[\|\nabla_{\ccalH_{k}}&\ell(Y,\bbPhi(X;\ccalH_k,\bbW))-\nabla_{\ccalH}\ell(Y_n,\bbPhi(X_n;\ccalH,\bbW_n))\|]  \nonumber\\
	      & \leq	\|\nabla_{\ccalH} \ell(Y,\bbPhi(X;\ccalH_k,\bbW))\|%^2  /2 F^{2L} \sqrt{K}
		\end{align}
% 		\bal\label{eqn:thm2_condition}
% 		C\|\nabla_{\ccalH}\ell(Y_n,\bbPhi(X_n;\ccalH_k,\bbW_n))  \|^{-1}\leq \sqrt{n}
% 		\eal
        then the iterate generated by graph learning step \eqref{eqn:GNN_Learning_Step} satisfies
        \bal
        \mbE[\ell(Y,\bbPhi(X;\ccalH_{k+1},\bbW))]\leq\ell(Y,\bbPhi(X;\ccalH_{k},\bbW)).
        \eal
    \end{lemma}
	
	{Lemma \ref{lemma:martingale} states that if the norm of the difference between the gradients on the graph and the graphon is bounded by the norm of the gradient on the graphon, then the loss on the graphon can be decreased by taking steps on the graph. In conjuction with Theorem \ref{thm:grad_Approximation}, Lemma \ref{lemma:martingale} thus gives an upper bound for the number of nodes that needed to follow the learning direction on the graphon, implying that it is always possible to construct a decreasing sequence of loss values by taking steps on the sampled graphs. 
	
	The specific condition on the number of nodes is determined by the norm of the gradient of the loss on the graphon. The intuition behind this is that, as the GNN improves its performance, the value of the loss decreases, and so the magnitude of its gradient decreases as well. Alternatively, we can think of the rate of decrease of the graphon gradient as a measure of the difficulty of the the learning problem, to which Lemma \ref{lemma:martingale} allows us to set the number of nodes accordingly.
	
	%We have shown that the learning step on the graphon and on the graph are close. Now, it remains to show the practical implications of Theorem \ref{thm:grad_Approximation} for obtaining the solution of the graphon ERM problem \eqref{eqn:ERM}. If the expected difference between the gradients is small, the iterations generated by \eqref{eqn:GNN_Learning_Step} will be able to follow the direction of the true gradient on the graphon learning problem. 
	%But because the distance between gradients is inversely proportional to $n$, we need to strike a balance between obtaining a good approximation and minimizing the computational cost. 
	
	Our main result is stated in Theorem \ref{thm:WNN_learning}, which shows that Algorithm \ref{alg:WNNL} converges if the rate at which the graph grows satisfies the condition in \eqref{eqn:thm2_condition}.

	\begin{theorem}\label{thm:WNN_learning}
		%Consider t$\sum \eta_k =\infty$,$\sum \eta_k^2 \leq\infty$. Under Assumptions \ref{as1}-\ref{as7}, if the loss $\ell(Y_n,\Phi(\bbW_n,X_n))$ converges to a finite value, and the.
		Consider the ERM problem in \eqref{eqn:ERM} and let $\bbPhi(X;\ccalH,\bbW)$ be an $L$-layer WNN with $F_0=F_L=1$, and $F_{l}=F$ for $1\leq l \leq L-1$.  Let $c \in (0,1]$, $\epsilon>0$, step size $\eta<{\Anl}^{-1}$, with $\Anl=\AnWNN+\AWNN F^{2L} \sqrt{K}$ and assume that the graphon convolutions in all layers of this WNN have $K$ filter taps [cf. \eqref{eq:graphon_convolution}]. Let $\bbPhi(\bbx_n;\ccalH,\bbS_n)$ be a GNN sampled from $\bbPhi(X;\ccalH,\bbW)$ as in \eqref{eqn:gcn_obtained}. Consider the iterates generated by equation \eqref{eqn:GNN_Learning_Step}, under Assumptions AS\ref{as1}-AS\ref{as7}, if at each step $k$ the number of nodes $n$ verifies 
% 		\bal\label{eqn:thm2_condition}
% 		C\|\nabla_{\ccalH}\ell(Y_n,\bbPhi(X_n;\ccalH_k,\bbW_n))  \|^{-1}\leq \sqrt{n}
% 		\eal
% 	\begin{align}\label{eqn:thm2_condition}
%     &\gamma c +\ccalO\bigg( \sqrt{\frac{\log(n^{3/2})}{n}}\bigg)\nonumber \\
%     &< \frac{1-\Anl\eta-\epsilon}{2} \|\nabla_{\ccalH} \ell(Y_n,\bbPhi(X_n;\ccalH_k,\bbWn)\|
%     \end{align}
%     then in finite time we will achieve an iterate $k^*$ such that the coefficients $\ccalH_{k^*}$ satisfy
%     \begin{align}\label{eqn:them2_claim}
%     \mbE_\ccalD[\|\nabla_{\ccalH}\ell(Y,\bbPhi(X;\ccalH_{k^*},\bbW))\|]\leq \gamma c+\epsilon, \quad 
%     \end{align} 
    \begin{align}\label{eqn:thm2_condition}
	      \mbE[\|\nabla_{\ccalH_{k}}&\ell(Y,\bbPhi(X;\ccalH_k,\bbW))-\nabla_{\ccalH}\ell(Y_n,\bbPhi(X_n;\ccalH,\bbW_n))\|]  \nonumber\\
	      & +\epsilon < 	\|\nabla_{\ccalH} \ell(Y,\bbPhi(X;\ccalH_k,\bbW))\|%^2  /2 F^{2L} \sqrt{K}
	\end{align}
    then Algorithm \ref{alg:WNNL} converges to an $\epsilon$-neighborhood of the solution of the Graphon Learning problem \eqref{eqn:ERM} in at most $k^*=\ccalO(1/\epsilon^2)$ iterations, where $\gamma$ is a constant that depends on the number of layers $L$, features $F$, and filter taps $K$ of the GNN [cf. Definition \ref{def:Constant_Of_GNN} in the Appendix \ref{sec:AppendixA}].
	\end{theorem}
\begin{proof} For every $\epsilon>0$, we define the stopping time $k^*$ as
\begin{align}
    k^*:=\min_{k\geq 0}\{\mbE_\ccalD[\|\nabla_{\ccalH} \ell(Y,\bbPhi(X;\ccalH_k,\bbW))\|]\leq  \gamma c+\epsilon \}.
\end{align}
Given the iterates at $k=k^*$ and the initial values at $k=0$, we can express the expected difference between the loss $\ell$ as the summation over the difference of iterates,
\begin{align}
    &\mbE[\ell(Y,\bbPhi(X;\ccalH_{0},\bbW))-\ell(Y,\bbPhi(X;\ccalH_{k^*},\bbW))]=\nonumber\\
    &\mbE\left[\sum_{k=1}^{k^*}\ell(Y,\bbPhi(X;\ccalH_{k-1},\bbW))-\ell(Y,\bbPhi(X;\ccalH_{k},\bbW)\right] \text{.} \nonumber
\end{align}
    Taking the expected value with respect to the final iterate $k=k^*$, we get
\begin{align}
    &\mbE\bigg[\ell(Y,\bbPhi(X;\ccalH_{k^0},\bbW))-\ell(Y,\bbPhi(X;\ccalH_{k^*},\bbW))\bigg]\nonumber\\
    &=\mathop{\mbE}_{k^*}\bigg[\mbE\bigg[\sum_{k=1}^{k^*}\ell(Y,\bbPhi(X;\ccalH_{k-1},\bbW))-\ell(Y,\bbPhi(X;\ccalH_{k},\bbW)\bigg]\bigg]\nonumber\\
    &=\sum_{t=0}^\infty \mbE\bigg[\sum_{k=1}^{t}\ell(Y,\bbPhi(X;\ccalH_{k-1},\bbW))\nonumber\\
    &\quad\quad\quad-\ell(Y,\bbPhi(X;\ccalH_{k},\bbW)\bigg]P(k^*=t) \text{.}\label{eqn:lemma6_law_of_total_probability}
\end{align}
Lemma \ref{lemma:martingale} applied to any $k\leq k^*$ verifies
\begin{align}
    &\mbE\bigg[\ell(Y,\bbPhi(X;\ccalH_{k-1},\bbW))-\ell(Y,\bbPhi(X;\ccalH_{k},\bbW))\bigg]\nonumber\geq \eta \gamma \epsilon^2 \text{.}
\end{align}
Coming back to \eqref{eqn:lemma6_law_of_total_probability}, we get
\begin{align}
    \mbE\bigg[\ell(Y,\bbPhi(X;\ccalH_{k^0},&\bbW))-\ell(Y,\bbPhi(X;\ccalH_{k^*},\bbW))\bigg]\nonumber\\
    &\geq \eta\gamma \epsilon^2 \sum_{t=0}^\infty t P(k^*=t)= \eta \gamma \epsilon^2 \mbE[k^*] \text{.}\nonumber
\end{align}
Since the loss function $\ell$ is non-negative, 
\begin{align}
    \frac{\mbE\bigg[\ell(Y,\bbPhi(X;\ccalH_{k^0},\bbW))\bigg]}{ \eta \gamma \epsilon^2 }
    &\geq  \mbE[k^*], \nonumber
\end{align}
from which we conclude that $k^* =\ccalO(1/\epsilon^2)$.
\end{proof}

\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/flocking/flocking10.pdf}
         \caption{Starting with $10$ nodes}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/flocking/flocking20.pdf}
         \caption{Starting with $20$ nodes}
     \end{subfigure}
	\caption{Velocity variation of the flocking problem for the whole trajectory in the testing set relative to the centralized controller.}
	\label{fig:flocking}
\end{figure*}

%Theorem \ref{thm:WNN_learning} presents the conditions under which Algorithm \ref{alg:WNNL} converges. 
The condition in \eqref{eqn:thm2_condition} implies that the rate of decrease in the norm of the gradient of the loss on the GNN
%of the loss function computed on the graph neural network 
needs to be slower than roughly $n^{-1/2}$. If the norm of the gradient does not vary between iterations, the number of nodes does not need to be increased.
We also see that the convergence of the gradient on the graphon given by Theorem \ref{thm:grad_Approximation} is equal to the bias term in \eqref{eq:thm_1} plus a constant $\epsilon$. We can keep increasing the number of nodes---and thus decreasing the bias---until the norm of the GNN gradient is smaller than the nontransferable constant value. Once this point is attained, there is no gain in decreasing the approximation bound any further \cite{ajalloeian2020analysis}. Recall that the constant term can be made as small as desired by tuning $c$, at the cost of decreasing the approximation bound. Further, note that assuming smoothness of the GNN is a mild assumption \cite{scaman2018lipschitz,jordan2020exactly,latorre2020lipschitz,fazlyab2019efficient,tanielian2021approximating,du2019gradient}. A characterization of the Lipschitz constant is out of the scope of this work. 
%In Algorithm \ref{alg:WNNL} we implement the desired behavior. By increasing the size of the graph $\bbG_n$ at every epoch, we are able to follow the gradient on the graphon learning problem. The advantage of Algorithm \ref{alg:WNNL} versus number of nodes fixed is twofold. 

% \red{
% \subsection{Discussion}
% \label{subsec:Discussion}
% L: I believe that this subsection is redundant and unnecessary. I would remove it. If there are things being said here that you didn't said in the paragraphs after each lemma/theorem, you can add them there.

% {In this section we have introduced three main theoretical contributions that support the idea of training on growing graphs. First, we introduced Theorem \ref{thm:grad_Approximation}, which quantifies the distance between the norm on the graphon, and the norm on the graph as a function of the number of nodes. Second, we are able to construct a decreasing sequence on the loss on the graphon by setting the minimum number of nodes needed to follow the learning direction. We then introduce an Algorithm that increases the number of nodes as we learn, the intuition being that as the GNN improves, the gradient of the loss on the graphon decreases, which requires a better approximation between the gradients. Third, we show that Algorithm \ref{alg:WNNL} converges to a neighborhood of the first order stationary point of the graphon learning problem in finite time. 
% } 
% }





==> TSP - Learning by transference/05-Numericals.tex <==

\section{Numerical Results}
\label{sec:Numericals}

%\subsection{Decentralized Control}
%\label{subsec:flocking}

%\input{figures/fig_snapshots.tex}

%A decentralized controller only relies on local information provided by other adjacent agents in the network. 

In this section we consider the problem of coordinating a set of $n$ agents initially flying at random to avoid collisions, and to fly at the same velocity. Also known as flocking, at each time $t$ agent $i$ knows its own position $r_i(t)\in \reals^2$, and speed $v_i(t)\in\reals^2$, and reciprocally exchanges it with its neighboring nodes if a communication link exists between them. Links are govern by physical proximity between agents forming a time varying graph $\bbG_n=(\ccalV,\ccalE)$. A communication link exists if the distance between two agents $i,j$ satisfies 
\begin{align}
    r_{ij}(t)=\|r_i(t)-r_j(t)\|\leq R=2m.
\end{align}
We assume that at each time $t$ the controller sets an acceleration $u_i \in [-10,10]^2$, and that it remains constant for a time interval $T_s=20ms$. The system dynamics are govern by,
\begin{align}
    r_i(t+1)&=u_i(t)T_s^2/2+v_i(t)T_s+r_i(t)\\
    v_i(t+1)&=u_i(t)T_s+v_i(t).
\end{align}
To avoid the swarm of robots to reach a null common velocity, we initialize the velocities at random $\bbv(t)=[v_1(t),\dots,v_n(t)]$, by uniformly sampling a common bias velocity $v_{BIAS}\sim \ccalU[-3,3]$, and then adding independent uniform noise $\ccalU[-3,3]$ to each agent.  The initial deployment is randomly selected in a circle always verifying that the minimum distance between two agents is larger than $0.1m$. On the one hand, agents pursue a common average velocity $\bar\bbv=(1/n)\sum_{i=1}^n v_i(t)$, thus minimizing the velocity variation of the team. On the other hand, agents are required to avoid collision. We can thus define the velocity variation of the team
\begin{align}
\sigma_{\bbv(t)}=\sum_{i=1}^{n}\|v_i(t)-\bar \bbv(t)\|^2,
\end{align}
and the collision avoidance potential 
\begin{align*}
\begin{split}
CA_{ij}=\begin{cases}
	\frac{1}{\|r_i-r_j\|^2}-\log(\|r_i-r_j\|^2) & \text{if $\|r_i-r_j\| \leq R_{CA}$}\\
	\frac{1}{R_{CA}^2}-\log(R_{CA}^2) & \text{otherwise,}
\end{cases} 
\end{split}
\end{align*}
with $R_{CA}=1m$. A centralized controller can be obtain by $u_i(t)^*=-n(v_i-\bar \bbv)+\sum_{j=1}^n\nabla_{r_i}CA(r_i,r_j)$ \cite{tanner2003stable}.

Exploiting the fact that neural networks are universal approximators \cite{barron1993universal,hornik1991approximation}, \textit{Imitation learning} can be utilized as a framework to train neural networks from information provided by an expert \cite{ross2011reduction,ross2010efficient}. Formally, we have a set of pairs $\ccalT= \{ \bbx_{m},\bbu^*_{m} \},m=1,\dots,M$, and during training we minimize the mean square error between the optimal centralized controller, and the output of our GNN $\|\bbu^*_{m}-\bbPhi(\bbx_m;\ccalH,\bbS)\|^2$. Denoting $\ccalN_i(t)$ the neighborhood of agent $i$ at time $t$, the state of the agents $\bbx(t)=[x(t)_{1},\dots,x(t)_{n}], x_i(t)\in \reals^6$, is given by
$$
x_i(t)=\sum_{j:j\in \ccalN_i(t)}\bigg[v_i(t)-v_j(t),\frac{r_{ij}(t)}{\|r_{ij}(t)\|^4},\frac{r_{ij}(t)}{\|r_{ij}(t)\|^2}\bigg]\text{.}
$$
Note that state $x_i(t)$, gets transmitted between agents if a communication link exists between them. 

In Figure \ref{fig:flocking} we can see the empirical manifestation of the claims we put forward. First and foremost, we are able to learn a GNN that achieves a comparable performance while taking steps on a smaller graphs. As seen in Figure \ref{fig:flocking}, GNNs trained with $n_0=\{10,20\}$ agents in the first epoch and adding $10$ agents per epoch (green line) are able to achieve a similar performance when reaching $100$ agents than the one they would have achieved by training with $100$ agents the same number of epochs. Besides, if we add less nodes per epoch, we are able to achieve a similar performance that we would have achieved by training on the large network for $30$ epochs. %We are also able to conclude that the initial number of nodes required for the algorithm to be used can be as small as a tenth of the size of the larger graph.


==> TSP - Learning by transference/figures/drawing/gradient.tex <==
\begin{tikzpicture}[scale=1,domain=-0.1:5]    

    %\node [below] at (0,0) {Goal};
    %\fill[rounded corners,draw=black,fill=black!75] (4,2) -- (5.73,3) -- (5.23,3.86) -- (3.5,2.86) --  cycle;
    \fill[draw=black!50,thick, fill=gray!50] (3,1) circle (1);

    %Arcs
    % the z line y0=0.578*x0+0.312
    

	\node [gray,below] at (8.2,2){ $\mbE[\|\nabla_{\ccalH}\ell(Y,\bbPhi(X;\ccalH_k,\bbW))-\nabla_{\ccalH}\ell(Y_n,\bbPhi(X_n;\ccalH_k,\bbW_n))\|]$};
	\node [red,below] at (0,1.1){ $\nabla_{\ccalH}\ell(Y,\bbPhi(X;\ccalH_k,\bbW))$};
	\node [blue,left] at (0,0){ $\ccalH_k$};
	\node [blue,above] at (3,1){ $\ccalH_{k+1}$};
	\fill[fill=blue] (3,1) circle (0.05); 
    \draw[red,->,very thick] (0,0) -- (3,1) node[right]{} ;
    \draw[gray] (3,1) -- (3+0.70,1+0.70) node[right]{} ;
        \fill[fill=blue] (0,0) circle (0.05); 
\end{tikzpicture}


==> TSP - Learning by transference/latex_resources/my_sections.tex <==
\usepackage{needspace}

% \nbsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsection}[1]{\needspace{1\baselineskip}\color{white}\medskip\subsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsection\quad #1.}}



% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\medskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}



==> TSP - Learning by transference/latex_resources/plot_appearance.tex <==


% This command sets the appearance of axis on pgfplots
\pgfplotsset{ ylabel near ticks,                 % Make x axis label appear close to figure
              xlabel near ticks,                 % Make y axis label appear close to figure
              tick label style = {font=\tiny},   % Write numbers in tiny font
              label style = {font=\tiny},        % Write axes labels in tiny size font
              title style = {font=\tiny},        % Write figure titles in tiny size font
            }

% style to draw dots in comb plots 
\tikzstyle{dot}          =[circle, draw=none, inner sep=0pt, minimum size =1.5mm, fill=black]
\tikzstyle{red dot}      =[dot, fill=red]
\tikzstyle{blue dot}     =[dot, fill=blue ]
\tikzstyle{red blue dot} =[dot, draw, thick, minimum size =1.2mm, red, fill=blue]
\def \greenfill {mygreen!40}

==> TSP - Learning by transference/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> figures/drawing/gradient.tex <==
\begin{tikzpicture}[scale=1,domain=-0.1:5]    

    %\node [below] at (0,0) {Goal};
    %\fill[rounded corners,draw=black,fill=black!75] (4,2) -- (5.73,3) -- (5.23,3.86) -- (3.5,2.86) --  cycle;
    \fill[draw=black!50,thick, fill=gray!50] (3,1) circle (1);

    %Arcs
    % the z line y0=0.578*x0+0.312
    

	\node [gray,below] at (8.2,2){ $\mbE[\|\nabla_{\ccalH}\ell(Y,\bbPhi(X;\ccalH_k,\bbW))-\nabla_{\ccalH}\ell(Y_n,\bbPhi(X_n;\ccalH_k,\bbW_n))\|]$};
	\node [red,below] at (0,1.1){ $\nabla_{\ccalH}\ell(Y,\bbPhi(X;\ccalH_k,\bbW))$};
	\node [blue,left] at (0,0){ $\ccalH_k$};
	\node [blue,above] at (3,1){ $\ccalH_{k+1}$};
	\fill[fill=blue] (3,1) circle (0.05); 
    \draw[red,->,very thick] (0,0) -- (3,1) node[right]{} ;
    \draw[gray] (3,1) -- (3+0.70,1+0.70) node[right]{} ;
        \fill[fill=blue] (0,0) circle (0.05); 
\end{tikzpicture}


==> latex_resources/my_sections.tex <==
\usepackage{needspace}

% \nbsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsection}[1]{\needspace{1\baselineskip}\color{white}\medskip\subsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsection\quad #1.}}



% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\medskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}



==> latex_resources/plot_appearance.tex <==


% This command sets the appearance of axis on pgfplots
\pgfplotsset{ ylabel near ticks,                 % Make x axis label appear close to figure
              xlabel near ticks,                 % Make y axis label appear close to figure
              tick label style = {font=\tiny},   % Write numbers in tiny font
              label style = {font=\tiny},        % Write axes labels in tiny size font
              title style = {font=\tiny},        % Write figure titles in tiny size font
            }

% style to draw dots in comb plots 
\tikzstyle{dot}          =[circle, draw=none, inner sep=0pt, minimum size =1.5mm, fill=black]
\tikzstyle{red dot}      =[dot, fill=red]
\tikzstyle{blue dot}     =[dot, fill=blue ]
\tikzstyle{red blue dot} =[dot, draw, thick, minimum size =1.2mm, red, fill=blue]
\def \greenfill {mygreen!40}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

